AI-based Aortic Vessel Tree Segmentation for Cardiovascular Diseases Treatment: Status Quo

The aortic vessel tree is composed of the aorta and its branching arteries, and plays a key role in supplying the whole body with blood. Aortic diseases, like aneurysms or dissections, can lead to an aortic rupture, whose treatment with open surgery is highly risky. Therefore, patients commonly undergo drug treatment under constant monitoring, which requires regular inspections of the vessels through imaging. The standard imaging modality for diagnosis and monitoring is computed tomography (CT), which can provide a detailed picture of the aorta and its branching vessels if completed with a contrast agent, called CT angiography (CTA). Optimally, the whole aortic vessel tree geometry from consecutive CTAs is overlaid and compared. This allows not only detection of changes in the aorta, but also of its branches, caused by the primary pathology or newly developed. When performed manually, this reconstruction requires slice by slice contouring, which could easily take a whole day for a single aortic vessel tree, and is therefore not feasible in clinical practice. Automatic or semi-automatic vessel tree segmentation algorithms, however, can complete this task in a fraction of the manual execution time and run in parallel to the clinical routine of the clinicians. In this paper, we systematically review computing techniques for the automatic and semi-automatic segmentation of the aortic vessel tree. The review concludes with an in-depth discussion on how close these state-of-the-art approaches are to an application in clinical practice and how active this research field is, taking into account the number of publications, datasets and challenges.

==> old_tab_2.tex <==
\begin{sidewaystable*}[ph!]
\centering
\caption{\tem{List of published studies related to computer-aided diagnosis, treatment, visualization and simulation of AD:
CFD: computational fluid dynamics;
CNN: convolutional neural network;
CT: computed tomography;
CTA: computed tomography angiography; 
FSI: fluid-structure interaction;
GFSC: greedy fine structure completion;
GVF: gradient vector flow;
MDCT: multi-detector CT;
MRI: magnetic resonance imaging.}}
%
\begin{tabular}[t]{lccc}
\hline
Publication & Methodology & Dataset  & Comments \\
\hline
%
\tem{\cite{Alimohammadi2014EvaluationOT}} & \tem{CFD} & \tem{CTA} & \tem{Virtual device deployment in AD}  \\
%
\tem{\cite{Bumler2020FluidstructureIS}} & \tem{FSI} & \tem{CTA} & \tem{Simulation of AD} \\
%
\tem{\cite{Bazilevs2009ComputationalFI}} & \tem{FSI} & \tem{CT (surface geometry)} & %
%
\tem{Simulation of the fontan configuration}\\
%
\tem{\cite{Bazilevs2010FromIT}} & \tem{FSI, CFD} & \tem{MRI, CT (surface geometry)} & \tem{Review}  \\
%
\tem{\cite{Bucurenciu2019StudyOA}}& \tem{Commercial software} &\tem{CTA} & \tem{Chronic TBAD, TL and FL segmented}      \\
%
\tem{\cite{Burris_2017}} & \tem{Vascular deformation mapping} & \tem{CTA} & \tem{Intra-patient mapping and visualization}\\
%
%%% SIMULATION - MALTE - BEGIN
\tem{\cite{Chen2013APS}} & \tem{CFD} & \tem{CTA} & \tem{Blood flow in AD}  \\
%
\tem{\cite{Crosetto2011FluidstructureIS}} & \tem{FSI} & \tem{MRI} & \tem{Simulation of aorta} \\
\cite{Dehghan2017Automatic} & Hessian matrix & \tem{E}nhanced CT & AD \tem{d}etection \\
%
\tem{\cite{deHoon_2014}} & \tem{CFD, flow visualization} & \tem{MRI} & \tem{Simulation-enhanced 4D MRI flow}\\
%
\cite{Duan2018AutomaticAD}  & GVF \tem{s}nake \tem{m}odel & CT & AD \tem{d}etection \\
%
\cite{inproceedings}           & Active-contour model & CTA &  Dissected aorta inner and outer wall extraction\\
%
\cite{Gayhart2013Automated} & Fast \tem{c}ircle \tem{d}etection & \tem{E}nhanced CT & AD \tem{d}etection \\
%
\cite{Harris2019}           & 2D CNN & \tem{E}nhanced CT & AD \tem{d}etection \\
%
\cite{Krissian2014Semi}& Level-set methods & MDCT & Intimal \tem{f}lap \tem{s}egmentation\\
%
\cite{Lohou2014Intimai}& Morphological operators & CTA & Intimal \tem{f}lap \tem{s}egmentation\\
%
\tem{\cite{Lohou2011Detection}} & 3D hole filling & \tem{E}nhanced CT & Intimal \tem{t}ear \tem{d}etection \\
%\tem{\cite{Bucurenciu2019StudyOA}}& \tem{commercial software to create geometry} &\tem{pre-,post- operative and follow-up aorta CTs} & \tem{Chronic TBAD, TL and FL segmented}      \\
%
\tem{\cite{Menichini2018ACM}} & \tem{CFD} & \tem{CTA} & \tem{Thrombus formation in AD}  \\
%
\tem{\cite{Mistelbauer_2016}} & \tem{Ad hoc, 2D plots} & \tem{CTA} & \tem{Comprehensive clinical visualization}\\
%
\cite{Morariu2014PolarBasedAS} & Polar-based  & CTA & Dissected aorta segmentation \\
%
\tem{\cite{Morariu2014Graph}}        & \tem{Graph-based}  & \tem{CTA} & \tem{Dissected aorta segmentation} \\
%
\cite{Morariu2015Extraction}&Spectral phase analysis & \tem{CTA} & Intimal \tem{f}lap \tem{s}egmentation \\
\cite{Morariu2016A} & GFSC & \tem{CTA} & Intimal \tem{f}lap \tem{s}egmentation\\
\cite{Morariu2016Increasing}& Phase congruency & \tem{CTA} & Intimal \tem{f}lap \tem{s}egmentation\\
\cite{Morariu2016Unsupervised}& Template filter and fuzzy c-means& CTA & Intimal \tem{f}lap \tem{s}egmentation\\
%
\tem{\cite{Qi_2016}} & \tem{Virtual intravascular endoscopy} & \tem{CTA} & \tem{Intimal tear visualization}\\
%
\tem{\cite{Qiao2019NumericalSO}} & \tem{FSI} & \tem{CTA} & \tem{Simulation of AD} \\
%
%\tem{\cite{Villiers2018AVP}} & \tem{FSI} & \tem{4D MRI} & \tem{arteriovenous fistula simulation}  \\
% not aorta but cerebral\tem{\cite{Ryu2009HighRW}} \\
%
%\tem{\cite{masterthesis}}\\
%\tem{\cite{Mao2008NormalTA}} \\
%\tem{\cite{Paruchuri2015AorticSD}} \\
%\tem{\cite{book}} & \tem{FEM} & \tem{Cylindrical tube} & \tem{AD propagation simulation} \\
%%% SIMULATION - MALTE - END
%\tem{\cite{Dotter1950AorticLA}*} & \tem{Statistical analysis} & \tem{Angiocardiography} & \tem{Aortic length measurement}\\
%\tem{\cite{Demertzis2010AorticAM}*} & \tem{3D multiplanar reconstruction} & \tem{CTA} & \tem{Aortic arch anatomy measurement}\\
%\tem{\cite{Demertzis2010AorticAM}*} & \tem{Multiplanar reconstruction} & \tem{CTA} & \tem{Aortic arch measurement}\\
%\tem{\cite{Renalarteryanatomy}*} & \tem{Quantitative vascular analysis} & \tem{Invasive selective angiography} & \tem{Renal artery anatomy measurement}\\
%\tem{\cite{Renalarteryanatomy}*} & \tem{vascular analysis} & \tem{Invasive selective angiography} & \tem{Renal artery measurement}\\
%\tem{\cite{Szpinda2012TheNG}*} & \tem{Anatomical dissection, digital-image analysis, regression analysis} & \tem{} & \tem{Common iliac arteries anatomy measurement}\\
%\tem{\cite{Szpinda2012TheNG}*} & \tem{regression analysis} & \tem{} & \tem{Common iliac arteries measurement}\\
%\tem{\cite{Olabarriaga2005SegmentationOT}*} & \tem{Nonparametric statistical grey level appearance modeling} & \tem{CTA} & \tem{Thrombus segmentation}\\
%\tem{\cite{Olabarriaga2005SegmentationOT}*} & \tem{appearance modeling} & \tem{CTA} & \tem{Thrombus segmentation}\\
%\tem{\cite{Shorten2019ASO}*} & \tem{Image data augmentation techniques and deep learning} \\ 
%\tem{\cite{Shorten2019ASO}*} & \tem{Deep Learning} \\ 
%\tem{\cite{Wong2016UnderstandingDA}*} & \tem{SVM, CNN} & \tem{Greyscale digit images} \\
%
\tem{\cite{Xiaojie2016}} & \tem{Spatial continuity prior model} & \tem{CTA} & \tem{Intimal \tem{f}lap \tem{s}egmentation} \\
\cite{Xu2019AnAD}  & \tem{CNN} & CTA & AD \tem{d}etection (Type A) \\
\hline
\end{tabular}
\label{table:table3}
%\end{table*}%
\end{sidewaystable*}
%\end{adjustbox}
